Dual-Time Smoothed Particle Hydrodynamics for Incompressible Fluid Simulation

In this paper we propose a dual-time stepping scheme for the Smoothed Particle Hydrodynamics (SPH) method. Dual-time stepping has been used in the context of other numerical methods for the simulation of incompressible fluid flows. Here we provide a scheme that combines the entropically damped artificial compressibility (EDAC) along with dual-time stepping. The method is accurate, robust, and demonstrates up to seven times better performance than the standard weakly-compressible formulation. We demonstrate several benchmarks showing the applicability of the scheme. In addition, we provide a completely open source implementation and a reproducible manuscript.

==> figures/cavity/cavity.tex <==
\begin{tabular}{lrrr}
\toprule
       Scheme &  nx &  Re &  CPU time (secs) \\
\midrule
   TVF, nx=50 &  50 & 100 &             0.13 \\
 DTSPH, nx=50 &  50 & 100 &             0.18 \\
  TVF, nx=100 & 100 & 100 &             0.14 \\
DTSPH, nx=100 & 100 & 100 &             0.20 \\
DTSPH, nx=150 & 150 & 100 &           450.65 \\
  TVF, nx=150 & 150 & 100 &          3097.82 \\
\bottomrule
\end{tabular}


==> figures/dam_break_2d/dam_break_2d.tex <==
\begin{tabular}{lr}
\toprule
      Scheme &  CPU time (secs) \\
\midrule
       DTSPH &            21.40 \\
        EDAC &            76.42 \\
$\delta$-SPH &            78.92 \\
\bottomrule
\end{tabular}


==> figures/dam_break_3d_old/dam_break_3d.tex <==
\begin{tabular}{lrr}
\toprule
Scheme & $\epsilon$ &  CPU time (secs) \\
\midrule
 DTSPH &      0.001 &           211.73 \\
 DTSPH &     0.0005 &           542.71 \\
 WCSPH &         NA &          3259.78 \\
\bottomrule
\end{tabular}


==> figures/elliptical_drop/elliptical_drop.tex <==
\begin{tabular}{lr}
\toprule
Scheme &  CPU time (secs) \\
\midrule
 DTSPH &            12.81 \\
 DTSPH &            78.88 \\
 DTSPH &           589.40 \\
  EDAC &          1108.66 \\
 WCSPH &          3625.50 \\
\bottomrule
\end{tabular}


==> figures/square_patch/square_patch_time.tex <==
\begin{tabular}{lrrr}
\toprule
       Scheme &  nx & $\epsilon$ &  CPU time (secs) \\
\midrule
 DTSPH, nx=50 &  50 &      0.001 &             3.76 \\
  EDAC, nx=50 &  50 &         NA &            24.03 \\
DTSPH, nx=100 & 100 &      0.001 &            29.78 \\
 EDAC, nx=100 & 100 &         NA &           193.72 \\
DTSPH, nx=200 & 200 &      0.001 &           247.32 \\
 EDAC, nx=200 & 200 &         NA &          1611.81 \\
\bottomrule
\end{tabular}


==> figures/taylor_green/beta/taylor_green.tex <==
\begin{tabular}{rr}
\toprule
Empty DataFrame
Columns: Index(['$\beta$', 'CPU time (secs)'], dtype='object')
Index: Int64Index([], dtype='int64') \\
\bottomrule
\end{tabular}

